Deep Policy Gradient Methods in Commodity Markets

The energy transition has increased the reliance on intermittent energy sources, destabilizing energy markets and causing unprecedented volatility, culminating in the global energy crisis of 2021. In addition to harming producers and consumers, volatile energy markets may jeopardize vital decarbonization efforts. Traders play an important role in stabilizing markets by providing liquidity and reducing volatility. Several mathematical and statistical models have been proposed for forecasting future returns. However, developing such models is non-trivial due to financial markets' low signal-to-noise ratios and nonstationary dynamics. This thesis investigates the effectiveness of deep reinforcement learning methods in commodities trading. It formalizes the commodities trading problem as a continuing discrete-time stochastic dynamical system. This system employs a novel time-discretization scheme that is reactive and adaptive to market volatility, providing better statistical properties for the sub-sampled financial time series. Two policy gradient algorithms, an actor-based and an actor-critic-based, are proposed for optimizing a transaction-cost- and risk-sensitive trading agent. The agent maps historical price observations to market positions through parametric function approximators utilizing deep neural network architectures, specifically CNNs and LSTMs. On average, the deep reinforcement learning models produce an 83 percent higher Sharpe ratio than the buy-and-hold baseline when backtested on front-month natural gas futures from 2017 to 2022. The backtests demonstrate that the risk tolerance of the deep reinforcement learning agents can be adjusted using a risk-sensitivity term. The actor-based policy gradient algorithm performs significantly better than the actor-critic-based algorithm, and the CNN-based models perform slightly better than those based on the LSTM.

==> duoforside.tex <==
%% Standard headers:

\DeclareOption{american}{\def \duo@lang {eng}}
\DeclareOption{english}{\def \duo@lang {eng}}
\DeclareOption{UKenglish}{\def \duo@lang {eng}}
\DeclareOption{USenglish}{\def \duo@lang {eng}}
\DeclareOption{norsk}{\def \duo@lang {bm}}
\DeclareOption{nynorsk}{\def \duo@lang {nn}}

\ExecuteOptions{norsk}
\ProcessOptions \relax


%% Initial code:

\RequirePackage{graphicx,keyval,xifthen}
\IfFileExists{type1cm.sty}{\RequirePackage{type1cm}}{}
\IfFileExists{type1ec.sty}{\RequirePackage{type1ec}}{}
\RequirePackage[T1]{url}


%% The main command:

\newcommand{\duoforside}[1][]{{%
  \parindent = 0pt   \parskip = 0pt
  \@ifundefined{hypersetup}{}{\hypersetup{pageanchor=false}}
  \setkeys{duo@keys}{#1}
  \duo@page@i
  \@ifundefined{duo@thesisname@eng}
    {\if@twoside \duo@blankpage \fi}
    {\duo@page@ii \duo@page@iii \duo@page@iv}
  \setcounter{page}{1}
  \@ifundefined{hypersetup}{}{\hypersetup{pageanchor=true}}
}}

\newcommand{\duo@empty}{}

\newcommand{\duo@page@i}{%
  \begin{titlepage}
    \fontfamily{\duo@font}\fontencoding{T1}
    \def \and {\\}
    \centering
    \fontsize{16}{19pt}\selectfont
    \null\par
    \vspace*{-2cm}
    {\fontsize{24}{28pt}\selectfont \duo@title\par}
    \vspace{1\baselineskip}
    \ifx \duo@subtitle = \duo@empty
    \else
        {\fontsize{20}{23pt}\fontshape{sl}\selectfont \duo@subtitle\par}
        \vspace{1\baselineskip}
    \fi
    \duo@author\par
    \vspace{1\baselineskip plus 3fill}
    \includegraphics[width=6cm]{DUO_UiO_segl}\par
    \vspace{1\baselineskip plus 4fill}
    \ifx \duo@kind = \duo@empty
    \else
      \duo@kind\par
      \vspace{1\baselineskip}
    \fi
    \ifx \duo@dept = \duo@empty
    \else
      \duo@dept\par
    \fi
    \ifx \duo@fac = \duo@empty
    \else
      \duo@fac\par
      \vspace{1\baselineskip}
    \fi
    \MakeUppercase{\csname duo@uio@\duo@lang\endcsname}\par
    \vspace{1\baselineskip}
    {\fontsize{12}{14pt}\selectfont \duo@date\par}
    \vspace{-2cm}
    \null
  \end{titlepage}
}

\newcommand{\duo@page@ii}{%
  \duo@blankpage
}

\newcommand{\duo@page@iii}{%
  \begin{titlepage}
    \def \and {\\}
    \centering
    \null\vfill
    {\fontsize{24}{28pt}\fontseries{bx}\selectfont \@title\par}
    \vfill
    {\fontsize{20}{23pt}\fontshape{sl}\selectfont \duo@subtitle\par}
    \vfill
    {\fontsize{16}{18pt}\selectfont \@author\par}
    \vfill\vfill\vfill
    \ifthenelse{\equal{\duo@image}{}}{}
      {\includegraphics[keepaspectratio,width=10cm,height=8cm]{\duo@image}\par\vfill\vfill}
  \end{titlepage}
}

\newcommand{\duo@page@iv}{%
  \begin{titlepage}
    \null
    \vfill
    \raggedright
    \def \and {, }
    \textcopyright~\arabic{duo@cur@year} \duo@author\\[\baselineskip]
    \leavevmode\duo@title\\[\baselineskip]
    \url{http://www.duo.uio.no/}
    \ifthenelse{\equal{\duo@printer}{}}{}
      {\\[\baselineskip] \csname duo@printertitle@\duo@lang \endcsname:
        \duo@printer}
  \end{titlepage}
}


%% The options:

\define@key{duo@keys}{author}{\def \duo@author {#1}}
\define@key{duo@keys}{date}{\def \duo@date {#1}}
\define@key{duo@keys}{dept}{\def \duo@dept {#1}}
\define@key{duo@keys}{fac}{\def \duo@fac {#1}}
\define@key{duo@keys}{image}{\def \duo@image {#1}}
\define@key{duo@keys}{kind}{\def \duo@kind {#1}}
\define@key{duo@keys}{long}[60]{\def \duo@sp {#1}}
\define@key{duo@keys}{nosp}[0]{\def \duo@sp {#1}}
\define@key{duo@keys}{option}{\def \duo@opt {(#1)}}
\define@key{duo@keys}{printer}{\def \duo@printer {#1}}
\define@key{duo@keys}{program}{\def \duo@program{#1}}
\define@key{duo@keys}{short}[30]{\def \duo@sp {#1}}
\define@key{duo@keys}{subtitle}{\def \duo@subtitle {#1}}
\define@key{duo@keys}{title}{\def \duo@title {#1}}

\newcommand{\duo@uio@eng}{University of Oslo}
\newcommand{\duo@uio@bm}{Universitetet i Oslo}
\newcommand{\duo@uio@nn}{Universitetet i Oslo}

\newcommand{\duo@fac@eng}{Faculty of mathematics and natural sciences}
\newcommand{\duo@fac@bm}{Det matematisk-naturvitenskapelige fakultet}
\newcommand{\duo@fac@nn}{Det matematisk-naturvitenskaplege fakultet}

\def \duo@author {\@author}
\providecommand{\duo@date}{\today}
\def \duo@dept {}
\def \duo@fac {\csname duo@fac@\duo@lang \endcsname}
\def \duo@image {}
\providecommand{\duo@kind}{}
\def \duo@opt {}
\def \duo@printer {Reprosentralen, \csname duo@uio@\duo@lang \endcsname}
\providecommand{\duo@program}{}
\def \duo@sp {60}
\def \duo@title {\@title}


%% Additional commands:

\newcommand{\subtitle}[1]{\def \duo@subtitle{#1}}
\subtitle{}


%% Find the best font:

\newcommand{\duo@font}{phv}  % Helvetica is always available, but use
\IfFileExists{t1ua1.fd}{\renewcommand{\duo@font}{ua1}}{} % Arial if possible.


%% Determine the term (as in "Spring 2016"):

\newcounter{duo@cur@year}   \setcounter{duo@cur@year}{\the\year}
\newcounter{duo@cur@month}  \setcounter{duo@cur@month}{\the\month}

\ifthenelse{\theduo@cur@month<7}
  {\newcommand{\duo@term@eng}{Spring}%
   \newcommand{\duo@term@bm}{V\aa ren}%
   \newcommand{\duo@term@nn}{V\aa ren}}
  {\newcommand{\duo@term@eng}{Autumn}%
   \newcommand{\duo@term@bm}{H\o sten}%
   \newcommand{\duo@term@nn}{Hausten}}
\newcommand{\duo@term}{\csname duo@term@\duo@lang\endcsname}
\newcommand{\duo@year}{\arabic{duo@cur@year}}


%% Other utilities:

\newcommand{\duo@blankpage}{%
    \thispagestyle{empty}
    \null
    \newpage}

\endinput

